How Do We Answer Complex Questions: Discourse Structure of Long-form Answers

Long-form answers, consisting of multiple sentences, can provide nuanced and comprehensive answers to a broader set of questions. To better understand this complex and understudied task, we study the functional structure of long-form answers collected from three datasets, ELI5, WebGPT and Natural Questions. Our main goal is to understand how humans organize information to craft complex answers. We develop an ontology of six sentence-level functional roles for long-form answers, and annotate 3.9k sentences in 640 answer paragraphs. Different answer collection methods manifest in different discourse structures. We further analyze model-generated answers -- finding that annotators agree less with each other when annotating model-generated answers compared to annotating human-written answers. Our annotated data enables training a strong classifier that can be used for automatic analysis. We hope our work can inspire future research on discourse-level modeling and evaluation of long-form QA systems.

==> figs/intro.tex <==
% \begin{figure}
% \begin{tikzpicture}
% \begin{axis}
% \addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=10, ymin=6, ymax=0] {figs/intro.png};
% \end{axis}
% \end{tikzpicture}
% \end{figure}

==> summary.tex <==

\section{Summarizing Long Form Answers}\label{sec:summary}
Lastly, we repurpose our role annotation dataset to summarize long form answers. Finding key sentences from long form answers has a practical appeal as users prefer concise answers~\cite{Choi2021DecontextualizationMS}. 
Our role annotations yield an extractive summarization dataset with 1K answer paragraphs in a new domain of long form answers, with 2.5 sentences marked as summary  by one or more annotators.
%\subsection{Experimental Setup}

\paragraph{Task / Data / Metric}
Given a question $q$ and its long form answer consisting of sentences $s_1, s_2,...s_n$, the goal is identifying a subset of sentences which can summarize the long form answer. 

We merge the answer paragraphs from two datasets and randomly split them into train, validation and test sets with a 70\%/15\%/15\% split.\footnote{We keep the split aligned with that of the role dataset.} We use all three annotations as gold summary during both training and evaluation, which yields a summarization dataset with multiple references. We therefore report \textit{weighted} precision, recall and F1 scores~\cite{Xu2016OptimizingSM}. The precise definition of our weighted metric can be found in \ref{subsec:append_sum_eval}. %This results in 724 (4523) / 156 (962) / 156 (992) answer paragraphs (sentences) in each split.


% We find identifying sentences corresponding to summary role is more subjective than the other roles as it has a notion of saliency (\ref{subsec:iaa}). Thus, instead of identifying a single gold summary sentence set, 
%\todo{FX: removed the previous sentence as the agreement is not bad} 

% \begin{align*} 
% p &=  \frac{\sum_{s_i}w_i \cdot y_i}{\sum_{s_i} y_i}\\ 
% r &= \frac{\sum_{s_i}w_i \cdot y_i }{\sum_{s_i}w_i} \\
% \end{align*}
% \ec{i'm not exactly sure this is how you computed, or how it should be computed... @fangyuan could you check?}
% Given a three-way annotation, we assign weight to each sentence based on how many annotator selected this sentence as summary. If any of the annotator selected this sentence as summary, the weight of the sentence equals to the number of annotators selected it as summary. Otherwise, we assign it a weight of three as all annotators label this as a non-summary sentence. 

%\subsection{Model}
% dd
\paragraph{Lower Bounds} We present two simple baselines, all taking a fixed number of sentences per paragraph, chosen from [1, 2, 3] based on the performance on validation set. (1) \textsc{Random}: A random set of three answer sentences (2) \textsc{Lead}: The lead three sentences of the paragraph. %(3) {Overlap}: The three sentences which have the highest unigram overlap with the question. 
% \todo{how many? we decide this on the dev set?} 
%\footnote{https://github.com/nlpyang/PreSumm.}
\paragraph{Models}  We use an extractive summarization model (PreSumm)~\cite{liu-lapata-2019-text} trained on the CNN/DailyMail dataset. PreSumm uses BERT to encode a document and outputs a score for each sentence to determine whether it belongs to the summary or not. We select the threshold of the score based on results on the validation set. We present results on the original model and the same model finetuned with our data. We use T5 to identify summary sentences as in role classification, only changing the categories from six-way roles to binary label. 
% finetune the model with our summary data. We report results on model which performs the best on the validation data.
% by continued training from the checkpoint of BertExt using the original set up from the paper

%except we have We fine-tune a T5 large model, by setting $role_{i}$ to be "Answer (Summary)" or "Others" based on whether answer sentence $i$ belongs to the summary.


% \todo{add implementation details}
% We explore two settings: (1) \textbf{PreSumm}: only using the answer paragraph as input (2) \textbf{PreSumm-question}: using the answer paragraph with the question prepended. We present results on the original PreSumm model as well as the same model finetuned with our data. \fy{presumm with question: todo}.

% \paragraph{Role models.}  We explore using the role model to identify summary classification. We take the role classification model with the highest F1 on "Answer (Summary)" (i.e. T5-large) and treat the sentences predicted to be "Answer (Summary)" as the summary sentence (\textbf{T5-role)}. We also report results on two other settings with the T5 model: (1) \textbf{T5-sum(partial)}: We train a T5-large model on the summaries in the role dataset (i.e. we collapse the label to be either "Answer (Summary)" or "Others"). This is denoted as partial as the role dataset contains a subset of the answer paragraphs from our summary dataset. (2) \textbf{T5-sum(full)}: Similarly, we train a T5-large model on the summaries in the summary dataset.

\paragraph{Human performance}  We approximate human performance with role annotation. Considering 3-way crowdsourced label as gold, we compute performance of summary annotation mapped from the role annotation by undergraduate annotators. We report results from two sets of summary sentences: (1) \textsc{Human (m)}: the set of sentence annotated as "Answer-Summary" by more than one annotator. (2) \textsc{Human (a)}: the set of sentence annotated as "Answer-Summary" by any annotator.
\paragraph{Result}
Table \ref{tab:summary_identification_results} reports results on summary task. Lead baseline shows strong performances as was in other domains. The model trained on CNN/Daily mail dataset~\cite{Hermann2015TeachingMT} outperforms lead baseline slightly, but falls behind the model fine-tuned on our dataset. The T5 model fine-tuned on our summary dataset performs the best. The results suggests a significant domain difference between newswire text (where lead is more prominent~\cite{liu-lapata-2019-text}) and long form answers. Thus, our dataset could support future research in extractive summarization across domains. %The model trained for fine-grained role classification also shows minor gains but finetuning just for summarization task shows the strongest performance among all. 
% \ec{perhaps we also report the number of sentences selected as a summary for each?} 

%Our task leaves a significant gap towards the human performance,
% We also report results on answer paragraphs with at least one summary sentence that is not in the first three sentences (total 515 answer paragraphs) in (Table \ref{tab:summary_identification_results_non_lead}). The human performance is computed with 267 samples and averaged across 3 annotators.
\begin{table}
\centering
\small
\begin{tabular}{lrrr}
\toprule
\textbf{System} & \ \textbf{P} &\ \textbf{R} & \ \textbf{F1}  \\ \midrule
Random & 0.36/0.35 & 0.57/0.58 & 0.46/0.44 \\%& 3/3 \\
%Overlap & 0.38/0.36 & 0.60/0.60 & 0.47/0.45 \\%& 3/3 \\ 
Lead & 0.41/0.42 & 0.65/0.69 & 0.50/0.52 \\%& 3/3 \\ \hline
PreSumm & 0.47/0.45 & 0.61/0.58 & 0.53/0.51 \\%&2.5/2.4\\ 
PreSumm-f & {0.47/0.47} & {\textbf{0.80}/\textbf{0.79}} & {0.59/0.59} \\%& {3.3/3.2}\\
% T5-role & 0.61/0.60 & 0.60/0.59 & 0.60/0.60 & 1.9/1.9\\
% T5-sum & \multirow{2}{*}{\textbf{0.63}/\textbf{0.66}} & \multirow{2}{*}{0.58/0.62} & \multirow{2}{*}{0.60/0.64}  & \multirow{2}{*}{1.8/1.8}\\
% (partial) & & &\\
T5-sum & \textbf{0.61/0.57} & {0.78/\textbf{0.79}} & {\textbf{0.68}/\textbf{0.66}}\\% & {2.6/2.6}\\
%Role$^'$ & \textbf{0.50}/\textbf{0.50} & 0.56/0.58 & 0.53/0.53 \\ \hline
% \multicolumn{3}{c}{Validation data}\\\hline
% PreSumm (finetuned) & 0.47 & \textbf{0.80} & \textbf{0.59} \\
% PreSumm & 0.47 & 0.60 & 0.53 \\
% Role & \textbf{0.50} & 0.55 & 0.53 \\
% Lead & 0.41 & 0.65 & 0.50 \\
% % PreSum-question & 0.39 & 0.62 & 0.48 \\
% Overlap & 0.37 & 0.60 & 0.46 \\
% Random & 0.36 & 0.59 & 0.45 \\
% \bottomrule
Human (a) & $0.64^*$ & $0.89^*$ & $0.74^*$\\% & $2.8^*$ \\
Human (m) & $0.82^*$ & $0.71^*$ & $0.76^*$\\% & $1.7^*$ \\
% Human (average) & $0.75^*$ & $0.69^*$ & $0.72^*$ &$1.8^*$ \\ 
\bottomrule
\end{tabular}
\caption{Summary identification result on validation and test answer paragraphs, presented as (val result/test result). $^*$Human number is computed on a subset.}\vspace{-0.4em}
\label{tab:summary_identification_results}
\end{table}

% \begin{table}
% \centering
% \begin{tabular}{l|l|l|l}
% \toprule
% \textbf{System} & \ \textbf{P} &\ \textbf{R} & \ \textbf{F1}   \\ \hline
% Human & 0.72 & 0.63 & 0.67  \\ \hline 
% Overlap-3 & 0.38 & \textbf{0.49} & \textbf{0.43} \\
% PreSum-question-3 & 0.35 & 0.46 & 0.40 \\
% PreSum-3 & 0.34 & 0.45 & 0.39 \\
% Overlap-2 & \textbf{0.40} & 0.35 & 0.37 \\
% Random-3 & 0.32 & 0.43 & 0.37 \\
% Lead-3 & 0.32 & 0.41 & 0.36 \\
% PreSum-question-2 & 0.36 & 0.32 & 0.34 \\
% PreSum-2 & 0.35 & 0.40 & 0.33 \\
% Random-2 & 0.32 & 0.28 & 0.30 \\
% Lead-2 & 0.31 & 0.28 & 0.30 \\ 
% \bottomrule
% \end{tabular}
% \caption{Summary identification result on 515 paragraphs with non-lead summary.}
% \label{tab:summary_identification_results_non_lead}(also sometimes called ``zones'')
% \end{table}
